Efficient Online Learning for Optimizing Value of Information: Theory and Application to Interactive Troubleshooting

We consider the optimal value of information (VoI) problem, where the goal is to sequentially select a set of tests with a minimal cost, so that one can efficiently make the best decision based on the observed outcomes. Existing algorithms are either heuristics with no guarantees, or scale poorly (with exponential run time in terms of the number of available tests). Moreover, these methods assume a known distribution over the test outcomes, which is often not the case in practice. We propose an efficient sampling-based online learning framework to address the above issues. First, assuming the distribution over hypotheses is known, we propose a dynamic hypothesis enumeration strategy, which allows efficient information gathering with strong theoretical guarantees. We show that with sufficient amount of samples, one can identify a near-optimal decision with high probability. Second, when the parameters of the hypotheses distribution are unknown, we propose an algorithm which learns the parameters progressively via posterior sampling in an online fashion. We further establish a rigorous bound on the expected regret. We demonstrate the effectiveness of our approach on a real-world interactive troubleshooting application and show that one can efficiently make high-quality decisions with low cost.

==> analysis_resampling.tex <==
\subsection{Analyzing the Cost of the Greedy Policy with Adaptively Re-sampled Posteriors}

We now consider the policy which greedily picks tests with respect to the adaptively-sampled posterior distribution of $H$ at each iteration.
% to adaptively enumerate new hypotheses after each iteration.
Denote the (re-)sampled distribution after performing $i$ tests as $\tilde{p}_i(H)$. Further, we use $\pi^g_{\tilde{p}_i}$ to denote the greedy policy (w.r.t. $\tilde{p}_i(H)$) after we have observed the outcome of the $i^{\text{th}}$ test. Assume $\pi^g_{\tilde{p}_i}$ picks test $e_i$ as the first test to perform, i.e., $\pi^g_{\tilde{p}_i}(\emptyset) = e_i$. By the tower rule of expectation, the expected cost of $\pi^g_{\tilde{p}_{i}}$ can be expanded as
\begin{align}
  & \cost(\pi^g_{\tilde{p}_{i}}) = \expctover{h}{\cost(\pi^g_{\tilde{p}_{i}}, h)} \nonumber \\
  =& \expctover{x_{e_{i}}} {\expctover{h}{ \cost(\pi^g_{\tilde{p}_{i}},h) \given x_{e_i}} } \nonumber \\
  =& 1 + \expctover{x_{e_{i}}} {\expctover{h}{ \cost(\pi^g_{\tilde{p}_{i}} \setminus \{x_{e_i}\},h) \given x_{e_i}} } \nonumber \\
  \stackrel{(a)}{\leq}& 1 + \expctover{x_{e_{i}}} {\left(2 \ln {1/\delta} + 1\right) \cost(\policy^* \given x_{e_i}) + (\eta_{\tilde{p}_i, x_{e_i}} + \delta) (T-1) } \label{eq:ub_nonadaptive}
  % &= 1 + \cost(\pi^g_{\tilde{p}_{i-1}} \given x_i)
\end{align}
Here $\eta_{\tilde{p}_i, x_{e_i}}$ denotes the fraction of hypothesis mass that is \emph{not} sampled by $\tilde{p}_i$ after observing $x_{e_i}$; by $\pi^g_{\tilde{p}_{i}} \setminus \{x_{e_i}\}$ we mean the policy $\pi^g_{\tilde{p}_{i}}$ excluding the first selected test (assuming that $\pi^g_{\tilde{p}_{i}}$ picks at least one test before it terminates); by $\cost(\policy^* \given x_{e_i})$ we mean the expected cost of (any arbitrary) policy $\pi^*$, conditioning on having observed $x_{e_i}$.
\begin{figure}[h]
  \centering
  \includegraphics[width=.5\textwidth]{fig/ada_s_policy.pdf}
  \caption{ Running policy $\pi^g_{\tilde{p}_{i}}$ starting from step $i$. On the left, we run $\pi^g_{\tilde{p}_{i}}$. If we replace (a) (i.e., all sub-trees starting from level $i+1$ as illustrated in the dashed rectangular box) by (b), then we are running greedy policy $\pi^g_{\tilde{p}_{i+1}}$ at step $i+1$ under a new sampled distribution $\tilde{p}_{i+1}$. % after running $\pi^g_{\tilde{p}_{i}}$ at step $i$.
    Since the resampled distribution covers more mass of $\cH$, by \thmref{thm:costupperbound_initalsamples} the policy on the right enjoys a better upper bound.}
  \label{fig:ada_s_policy}
\end{figure}

Now, instead of running greedy algorithm under $p_i$, we resample the posterior to cover more mass of $\cH$, and run $\pi^g_{\tilde{p}_{i+1}}$ afterwards based on the resampled posterior (see \figref{fig:ada_s_policy}). Denote such policy by $\pi^g_{i,\tilde{p}_{i}}@\pi^g_{\tilde{p}_{i+1}}$, we then have
\begin{align}
  &\cost(\pi^g_{i,\tilde{p}_{i}}@\pi^g_{\tilde{p}_{i+1}}) = 1 + \expctover{x_{e_{i}}} {\expctover{h}{ \cost(\pi^g_{\tilde{p}_{i+1}} \given x_{e_i}} } \nonumber \\
  \stackrel{(a)}{\leq}& 1 + \expctover{x_{e_{i}}} {\left(\ln {1/\delta} + 1\right) \cost(\policy^* \given x_{e_i}) + (\eta_{\tilde{p}_{i+1}, x_{e_i}} + \delta) (T-1) }. \label{eq:ub_1step_adaptive}
\end{align}
Since $\eta_{\tilde{p}_{i+1}, x_{e_i}} \leq \eta_{\tilde{p}_{i}, x_{e_i}}$, the upper bound in Equation~\eqref{eq:ub_1step_adaptive} is lower Equation~\eqref{eq:ub_nonadaptive}. Similarly, we can show that greedy policy $\pi^g_{1,\tilde{p}_{1}}@\pi^g_{2,\tilde{p}_{2}}@\dots$ with fully adaptively-resampled posteriors enjoys a better cost upper bound than the greedy policy $\pi^g_{1,\tilde{p}_{1}}$ with initial sampled prior only \footnote {Note that we only compare the derivable cost \emph{upper bound} as a qualitative measurement of the algorithms under different settings, and show that the cost of the algorithm with adaptive resampling has stronger upper bound. We \emph{do not} claim that with adaptive resampling it always incurs lower cost than the non-resampling version.}.

% \yuxin{Todo: prove that the greedy policy w.r.t. the resampled distribution is an $\frac{1}{1-\eta}$-greedy policy w.r.t. the initial sampled distribution -- or something like that...}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_sampling"
%%% End:


==> method_notes.tex <==

\section{Method}



\subsection{Sample from the probabilistic diagnostic matrix $S$} For
each root-cause $y_i \in \cY$, we can enumerate (or sample from) all
the possible realizations of the symptoms. Denote a specific full
realization of all tests in $\cT$ by $\bx_{\cT}$. Suppose that we have
observed the outcome of $t \in \cA$, then the posterior probability of
$h \equiv \bx_{\cT}$ can be computed as:

\begin{align}
  p(h \given \bx_{\cA}) % &= \sum_{y} p(h, y \given \bx_{\cA}) \\
                          &= \sum_{y} p(h \given y, \bx_{\cA}) p(y \given \bx_{\cA}) \nonumber \\
                          &= \sum_{y} p(\bx_{\cA},\bx_{\cT \setminus \cA} \given y, \bx_{\cA}) p(y \given \bx_{\cA}) \nonumber \\
                          &= \unit{\bx_{\cT} \sim \bx_{\cA}} \sum_{y} p(\bx_{\cT \setminus \cA} \given y) p(y\given \bx_{\cA}) \nonumber \\
                          &= \unit{\bx_{\cT} \sim \bx_{\cA}}
                            \frac{\sum_{y} p(y) p(\bx_{\cA} \given y) p(\bx_{\cT \setminus \cA} \given y) }
                            {\sum_y p(y) p(\bx_{\cA} \given y)} \nonumber \\
                            % &= \unit{\bx_{\cT} \sim \bx_{\cA}}
                            % \frac{\sum_{k} p(y_k) \prod_{i\in\cA} p(x_{i} \given y_k) \prod_{j \in \cT\setminus\cA} p(x_{j} \given y_k) }
                            % {\sum_y p(y) p(\bx_{\cA} \given y)} \\
                          &= \unit{\bx_{\cT} \sim \bx_{\cA}}
                            \frac{\sum_{y} p(y) p(\bx_{\cT} \given y)}
                            {\sum_y p(y) p(\bx_{\cA} \given y)} \label{eq:resampling} \\
                          &= \unit{\bx_{\cT} \sim \bx_{\cA}}
                            \frac{p(\bx_{\cT})}
                            {p(\bx_{\cA})} \nonumber
\end{align}
% or equivalently,
% \begin{align*}
%   p(h \given \bx_{\cA}) &= \unit{\bx_{\cT} \sim \bx_{\cA}} \cdot \frac{p(\bx_{\cA}, \bx_{\cT \setminus \cA}) }
%   {p(\bx_{\cA})}
% \end{align*}

After performing a new test $e$ and having observed $x_e$, we have
\begin{align}
  p(h \given \bx_{\cA\cup\{e\}}) &=  \unit{\bx_{\cT} \sim \bx_{\cA}} \unit{\bx_{\cT} \sim x_e}
                                   \frac{p(\bx_{\cT})} { p(\bx_{\cA}) } \frac{p(\bx_{\cA})}{p(\bx_{\cA \cup \{e\} })} \nonumber \\
                                 &=  p(h \given \bx_{\cA}) \unit{h \sim x_e} \frac{p(\bx_{\cA})}{p(\bx_{\cA \cup \{e\} })} \nonumber \\
                                 &\propto p(h \given \bx_{\cA}) \unit{h \sim x_e}\label{eq:hypupdate}
\end{align}
That is, suppose we have \textit{enumerated all hypotheses}, at each
iteration, we just need to remove the inconsistent hypotheses (and
normalize the weight to be posterior probability of each hypothesis).


If we only maintain samples of the hypotheses, then at each iteration,
we can \emph{resample} the hypotheses according to
Equation~\eqref{eq:resampling}.

\subsubsection{Resampling}

\paragraph{The naive approach (rejection sampling)} A practical way to
sample the hypotheses is as follows. Initially we sample enough
hypotheses from the probabilistic diagnostic matrix $S$, for example,
we can keep sampling new hypotheses till the cumulative probability of
the samples is $\geq 98\%$. For each (unique) sample we assign a
weight which equals its probability. Denote the total weight of the
samples by $W_0$. At each iteration $i$, we perform a new test $e_i$
and observe its outcome. Then we remove the inconsistent hypotheses
(according to Equation \eqref{eq:hypupdate}), and check if the total
weight of the remaining mass is less than $W_0/2$. If yes, the we
regenerate a new set of samples and set $W_0$ to be the total weights
of the new samples, otherwise we keep performing new tests.

At some point we can enumerate all the hypotheses, and hence we don't
need to resample from then on.

\paragraph{Enumerating the most probable hypotheses} Instead of randomly sampling hypotheses and discarding the least probable samples, we can enumerate the hypotheses with high probability only.
\begin{algorithm}[h]
  \caption{Enumerating the most probable hypotheses}\label{alg:enumhyp}
  \begin{algorithmic}
    \STATE {\bfseries Input:}  Conditional probability table $S = \{\theta_{ij}\}$, prior on root-causes $P_0(Y)$.
    \STATE {\bfseries Output:} Hypotheses set $H$.
    \STATE $H \leftarrow \emptyset$
    \FORALL {$y_i \in \{y_1, \dots, y_n\}$}
    \STATE $H_i \leftarrow \emptyset$, Max priority queue $Q_i \leftarrow \emptyset$, probability mass $m_i \leftarrow 0$
    \STATE Number of samples $n_i \leftarrow 0$
    \STATE Sort $(t_1, \dots, t_m)$ in descending order according to score function $s(t_i) = \max\{p(x_i = 1 \given y_i), p(x_i = 0 \given y_i) \}$. Save the original ordering of $t$'s to vector $\bd$.
    \STATE $\bb = (b_1,\dots, b_m) \leftarrow \{\argmax_{x_1} p(x_1 \given y_i), \dots, \argmax_{x_m} p(x_m \given y_i)\}$
    \STATE $\bc = (c_1,\dots, c_m) \leftarrow \{0, \dots, 0\}$
    \STATE $Q_i$.push$(\bc)$
    \WHILE {$m_i < M$ $\&\&$ $n_i < N$}
    \STATE $\bc = (c_1,\dots, c_m) \leftarrow Q_i .\text{top}()$,
    \STATE $Q_i .\text{pop}()$
    \STATE $H_i \leftarrow H_i \cup \{\bc\}$
    \STATE $C \leftarrow$ \textsf{FindCandidates}$(c_1,\dots, c_m)$
    \IF {$Q_i$ does not contain $\bc \in C$} \STATE $Q_i.\text{push}(\bc)$ \ENDIF
    \ENDWHILE
    \FORALL {$\bc \in H_i$}
    \STATE $\bh \leftarrow \bb \oplus \bc$
    \STATE Update $\bh$ according to the original ordering of tests $\bd$
    \STATE $H.\text{insert}(\bh)$
    \ENDFOR
    \ENDFOR
  \end{algorithmic}
\end{algorithm}

Here is the subroutine for finding the next candidate hypotheses to enumerate:

\begin{algorithm}[h]
  \caption{\textsf{FindCandidates}$(c_1,\dots, c_m)$}\label{alg:findncand}
  \begin{algorithmic}
    \STATE {\bfseries Input:}  binary vector $(c_1,\dots, c_m)$
    \STATE {\bfseries Output:}  a set of candidate vectors $C$
    \STATE $C \leftarrow \emptyset$
    \IF {$c_m = 0$ }
    \STATE $C \leftarrow C \cup \{(c_1, \dots, c_{m-1}, 1)\}$
    \ENDIF
    \STATE Find the last consecutive occurrence of 0,1 in $\bc$, denoted by $c_{\text{pos}} = 0 ,~c_{\text{pos+1}} = 1$
    \STATE $C \leftarrow C \cup \{ (c_1, \dots, c_{\text{pos}} \oplus 1, c_{\text{pos}+1} \oplus 1, \dots)\}$
  \end{algorithmic}
\end{algorithm}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_sampling"
%%% End:

